Learning Over-Parametrized Two-Layer ReLU Neural Networks beyond NTK

We consider the dynamic of gradient descent for learning a two-layer neural network. We assume the input $x\in\mathbb{R}^d$ is drawn from a Gaussian distribution and the label of $x$ satisfies $f^{\star}(x) = a^{\top}|W^{\star}x|$, where $a\in\mathbb{R}^d$ is a nonnegative vector and $W^{\star} \in\mathbb{R}^{d\times d}$ is an orthonormal matrix. We show that an over-parametrized two-layer neural network with ReLU activation, trained by gradient descent from random initialization, can provably learn the ground truth network with population loss at most $o(1/d)$ in polynomial time with polynomial samples. On the other hand, we prove that any kernel method, including Neural Tangent Kernel, with a polynomial number of samples in $d$, has population loss at least $\Omega(1 / d)$.

==> reduction.tex <==
\section{Learning ReLU Teacher Networks: A Reduction}\label{app_red}
  In this part we describe a simple reduction from learning ReLU target networks to learning the labeling function of equation \eqref{eq_abs}.
  Let $a \in \real^r$ and $W^{\star} \in \real^{r \times d}$ denote the weights of the output and input layers, respectively.
  For an input vector $x \in \real^d$ drawn from a distribution, denote by \[ y = {a}^{\top} \relu({W^{\star}} x). \]
  Consider solving the least squares regression with $(x, y)$.
  \begin{align*}
    z^{\star} = \argmin_{z \in \real^d} \exarg{x, y}{(z^{\top}x - y)^2}.
  \end{align*}

  \begin{proposition}\label{prop_relu_abs}
    Assume that $x \in \real^d$ is drawn from a symmetric distribution, that is, $\Pr(x) = \Pr(-x)$.
    Denote by $\hat{y} = 2(y - {z^{\star}}^\top x)$. Then $\hat{y}$ is generated  from $x$ according to equation \eqref{eq_abs} with weights $a$ and $W^{\star}$,
		\[ \hat{y} = a^{\top}\relu(W^{\star}x) + a^{\top}\relu(-W^{\star}x). \]
  \end{proposition}

  \begin{proof}
    We have that
    {\small\begin{align*}
      \exarg{x}{(z^{\top} x - y)^2} &= \exarg{x}{\left(z^{\top} x - \frac{{a}^{\top}W^{\star} x + {a}^{\top} \bigabs{W^{\star}x} } 2\right)^2} \\
      &= \exarg{x}{\Bracket{\inner{z - \frac {{a}^{\top} W^{\star}} 2}{x} - \frac{{a}^{\top}\bigabs{W^{\star}x}} 2}^2} \\
      &= \exarg{x}{\inner{z - \frac{{a}^{\top} W^{\star}} 2}{x}^2} - \exarg{x}{\inner{z - \frac{{a}^{\top}W^{\star}}{2}}{x} \frac{{a}^{\top} \bigabs{W^{\star}x}}{2}} + \exarg{x}{\frac {({a}^{\top} \bigabs{W^{\star}x})^2} 4}
    \end{align*}}
    By the assumption that $x$ is drawn from a symmetric distribution, we have that the second term is zero.
    Note that the third term is independent of $z$. Hence $z^{\star}$ is equal to ${a}^{\top} W^{\star} / 2$.
    This implies that
    \[ \hat y = 2y - 2\inner{{a}}{\frac {W^{\star}x} 2}
              = 2\inner{{a}}{\relu(W^{\star}x) - \frac{W^{\star}x} 2}
              = \inner{{a}}{{\relu(W^{\star} x) + \relu(-W^{\star}x)} }. \]

  \end{proof}
  Based on this reduction, we could therefore apply our result for learning target networks with ReLU activations.

